GSP = DSP + Boundary Conditions -- The Graph Signal Processing Companion Model

The paper presents the graph signal processing (GSP) companion model that naturally replicates the basic tenets of classical signal processing (DSP) for GSP. The companion model shows that GSP can be made equivalent to DSP 'plus' appropriate boundary conditions (bc) - this is shown under broad conditions and holds for arbitrary undirected or directed graphs. This equivalence suggests how to broaden GSP - extend naturally a DSP concept to the GSP companion model and then transfer it back to the common graph vertex and graph Fourier domains. The paper shows that GSP unrolls as two distinct models that coincide in DSP, the companion model based on (Hadamard or pointwise) powers of what we will introduce as the spectral frequency vector $\lambda$, and the traditional graph vertex model, based on the adjacency matrix and its eigenvectors. The paper expands GSP in several directions, including showing that convolution in the graph companion model can be achieved with the FFT and that GSP modulation with appropriate choice of carriers exhibits the DSP translation effect that enables multiplexing by modulation of graph signals.

==> images/auxiliar-sampling.tex <==


\section{Sampling in the Canonical Model}
\label{sec:sampling}
In this section, we briefly explore sampling in the canonical model. In \cite{shimoura-2021}, we explored the four steps of sampling in both vertex and spectral domains - subsampling, decimation, upsampling, interpolation.

Consider a signal $s$ that is bandlimited in the spectral domain with bandlimit $K < N$. Let $\delta$ be the sampling operator. The sampled signal is $\delta \odot s$ which chooses $K$ entries of $s$ and zeros out $N-K$ entries of $s$.

One main result for decimation in \cite{shimoura-2021} was the $K \times K$ decimated graph, $A_d = \textrm{GFT}_d^{-1} \Lambda_d \textrm{GFT}_d$. The decimated eigenvectors, $\textrm{GFT}_d^{-1}$ were found by taking an invertible block of the $\textrm{GFT}^{-1}$. The decimated eigenvalues were found by taking the $K$ chosen eigenvalues in $\delta \odot \lambda$. For more details, see \cite{shimoura-2021}.

We now verify the decimated graph $A_d$ using the companion model.

\subsection{Step 1: GSP Spectral Companion Model Decimation}
Consider a signal $s$ that is bandlimited in the $\left\{q_i\right\}$ spectral impulse representation with bandlimit $K$, $s\xrightarrow{\left(\mathcal{V}^*\right)^{-1}} q = \left[q^{K^T}, 0^T\right]^T$. For the spectral companion model, the vertex domain shift is $A_{\textrm{comp}} = \frac{1}{\sqrt{N}}\mathcal{V}^* \Lambda \sqrt{N}\mathcal{V}^{*^{-1}}$ and the spectral domain shift is $C_{\textrm{comp,sp}} = \sqrt{N}\mathcal{V}^{*^{-1}} \Lambda^* \frac{1}{\sqrt{N}}\mathcal{V}^*$ (See Remark \ref{subsec:dspcompanion}).

Following the process in \cite{shimoura-2021}, the decimated eigenvalues $\Lambda_{d,\textrm{comp}}$ are the $K$ chosen eigenvalues of $\Lambda$. The decimated eigenvectors is a $K
\: \times \: K$ block of $\mathcal{V}^*$. Since $q$ is bandlimited, the first $K$ columns of $\mathcal{V}^*$ are chosen. $\delta$ then chooses $K$ rows of those columns, producing a smaller Vandermonde matrix, $\mathcal{V}_d^*$. The Vandermonde matrix contains the conjugate of the decimated eigenvalues, $\Lambda_{d,\textrm{comp}}$ because $\delta$ chooses the rows in $\mathcal{V}^*$ corresponding to the decimated eigenvalues. So, $\textrm{GFT}^{-1}_d = \mathcal{V}^*_d$. Therefore, the decimated graph is $\frac{1}{\sqrt{N}}\mathcal{V}_d^* \Lambda_{d,\textrm{comp}} \sqrt{N}\mathcal{V}_d^{*^{-1}} = \frac{1}{\sqrt{K}}\mathcal{V}_d^* \Lambda_{d,\textrm{comp}} \sqrt{K}\mathcal{V}_d^{*^{-1}}$. The spectral domain shift is
$C_{\textrm{comp,sp,d}} = \sqrt{K}\mathcal{V}_d^{*^{-1}} \Lambda_{d,\textrm{comp}}^* \frac{1}{\sqrt{K}}\mathcal{V}^*$.

\begin{remark}
    In the case of uniform sampling in DSP, $C_{\textrm{comp,sp,d}}$ would be the decimated cycle graph. The boundary conditions (and Cayley-Hamilton Theorem) cause the characteristic polynomial and thus, the eigenvalues to not be the $N$ roots of unity. So, we do not obtain the DSP decimated cycle graph, even when uniformly sampling in the companion graph. The companion model decimation is equivalent to DSP with appropriate boundary conditions.
\end{remark}

\subsection{Step 2: GSP Vertex Domain Decimation}
If $\delta$ chooses complex conjugate pairs in $\Lambda_{d,\textrm{comp}}^*$\footnote{This condition is also true in DSP. When uniformly sampling, we always choose complex conjugate pairs. When not uniformly sampling, $C_{\textrm{comp,sp,d}}$ is not real.}, then $C_{\textrm{comp,sp,d}}$ is real and $C_{\textrm{comp,sp,d}}$ is the companion matrix for the decimated graph $A_d$ by \eqref{eqn:compsp}. This result is intuitively pleasing because sampling with the companion model is consistent with traditional GSP sampling, i.e., the companion model sampling yields a decimated companion graph, $C_{\textrm{comp,sp,d}}$, that is the companion graph for the decimated graph $A_d$ (See result \ref{res:shiftAspC}).

\subsection{Example}
We sample the 12 node directed ladder graph in figure \ref{fig:ladderdir12} with $\delta = [0,0,0,0,1,1,0,0,1,1,0,0]^T$. This chooses four of the eigenvalues: $.767 \pm .538j, .403 \pm .864j$ (shown in the top of figure \ref{fig:sampling}). Assuming the signal is bandlimited with bandlimit 4, this chooses the first four columns of the $\mathcal{V}^*$ and $\text{GFT}^{-1}$. The $\delta$ then chooses four of the rows. This is shown in the bottom of figure \ref{fig:sampling}. Observe that the chosen block of $\mathcal{V}^*$ is also a Vandermonde matrix with values: $.767 \pm .538j, .403 \pm .864j$.

Using these blocks, we find $A_d$, $M_d$, and $C_{\textrm{comp,sp,d}}$, shown in figure \ref{fig:sampling2}. We observe that $C_{\textrm{comp,sp,d}}$ is the companion matrix of $A_d$ and $M_d$ since they all have the same eigenvalues: $.767 \pm .538j, .403 \pm .864j$. Companion model sampling is consistent with traditional GSP sampling.

\begin{figure}[hbt!]
\begin{center}
	\includegraphics[width=5cm, keepaspectratio]{images/unitcircle.png}
	\includegraphics[width=4cm, keepaspectratio]{images/gftinvsampling.png}
 	\includegraphics[width=4cm, keepaspectratio]{images/vandermondesampling.png}
	\caption{The chosen eigenvalues (top) and small blocks of the $\textrm{GFT}^{-1}$ and $\mathcal{V}^*$ (bottom). The larger yellow box chooses columns because of the bandlimitedness. The red boxes choose rows based on $\delta$. The small block of $\mathcal{V}^*$ is also a Vandermonde matrix using the chosen eigenvalues.}
		\label{fig:sampling}
\end{center}
\end{figure}

\begin{figure}[hbt!]
\begin{center}
	\includegraphics[width=6cm, keepaspectratio]{images/companionsampling.png}
	\caption{The decimated graphs $A_d$, $M_d$, $C_{\textrm{comp,sp,d}}$. $C_{\textrm{comp,sp,d}}$ is the companion graph of $A_d$.}
		\label{fig:sampling2}
\end{center}
\end{figure}
